Improving Graph Neural Networks with Learnable Propagation Operators

Graph Neural Networks (GNNs) are limited in their propagation operators. In many cases, these operators often contain non-negative elements only and are shared across channels, limiting the expressiveness of GNNs. Moreover, some GNNs suffer from over-smoothing, limiting their depth. On the other hand, Convolutional Neural Networks (CNNs) can learn diverse propagation filters, and phenomena like over-smoothing are typically not apparent in CNNs. In this paper, we bridge these gaps by incorporating trainable channel-wise weighting factors $\omega$ to learn and mix multiple smoothing and sharpening propagation operators at each layer. Our generic method is called $\omega$GNN, and is easy to implement. We study two variants: $\omega$GCN and $\omega$GAT. For $\omega$GCN, we theoretically analyse its behaviour and the impact of $\omega$ on the obtained node features. Our experiments confirm these findings, demonstrating and explaining how both variants do not over-smooth. Additionally, we experiment with 15 real-world datasets on node- and graph-classification tasks, where our $\omega$GCN and $\omega$GAT perform on par with state-of-the-art methods.

==> images/Fig12.tex <==
%\iffalse
%\begin{figure*}
%    \includegraphics[  width=0.45\textwidth]{images/omegaImpulse4.png}
% 
%    \caption{The impulse response for different $\omega$ values.
%     }
%     \label{fig:omegaImpulse}
% \end{figure*}
% \fi
 
 
\begin{figure*}
\centering
\begin{minipage}{0.48\textwidth}
\begin{tikzpicture}
  \begin{axis}[
      width=1.0\linewidth, 
      height=0.6\linewidth,
      grid=major,
      grid style={dashed,gray!30},
      xlabel=Layers,
      ylabel=Accuracy (\%),
      ylabel near ticks,
      legend style={at={(0.2,0.625)},anchor=north,scale=1.0, draw=none, cells={anchor=west}, font=\tiny, fill=none},
      legend columns=1,
      xtick={0,1,2,3,4,5},
      xticklabels = {2,4,8,16,32,64},
      yticklabel style={
        /pgf/number format/fixed,
        /pgf/number format/precision=3
      },
      scaled y ticks=false,
      every axis plot post/.style={thick},
    ]
    \addplot[red, mark=oplus*, forget plot]
    table[x=layer,y=omegagcn,col sep=comma] {data/omegaGCNvsGCN_cora.csv};
    \addplot[blue, mark=oplus*, forget plot]
    table[x=layer,y=omegagcn,col sep=comma] {data/omegaGCNvsGCN_citeseer.csv};
    \addplot[red, style=dotted, mark=oplus*, forget plot]
    table[x=layer,y=gcn,col sep=comma] {data/omegaGCNvsGCN_cora.csv};
    \addplot[blue, style=dotted, mark=oplus*, forget plot]
    table[x=layer,y=gcn,col sep=comma] {data/omegaGCNvsGCN_citeseer.csv};
    \addplot[red, draw=none] coordinates {(1,1)};
    \addplot[blue, draw=none] coordinates {(1,1)};
    \addplot[gray, draw=none] coordinates {(1,1)};
    \addplot[gray, style=dotted, draw=none] coordinates {(1,1)};
    \legend{Cora, Citeseer, $\omega$GCN, GCN}
    \end{axis}
\end{tikzpicture}
\caption{GCN vs. $\omega$GCN. The accuracy of $\omega$GCN improves with more layers while GCN's degrades due to over-smoothing.}
\label{fig:omegaGCNvsGCN}
\end{minipage} \hspace{0.5em}
\begin{minipage}{.48\textwidth}
\centering
    \includegraphics[  width=1.0\textwidth]{images/omega_new.png}
    \caption{The impulse response of
    $\omega$GCN's spatial operator for different $\omega$ values. For $\omega=0.5,1.0$ we see non-negative weights, while for $\omega=1.5$ we see mixed-sign weights. The dashed node starts from a feature of 1 and the rest with 0.
     }
     \label{fig:omegaImpulse}


\end{minipage}
\end{figure*}
 
 
